3D Human Pose Estimation via Intuitive Physics

Estimating 3D humans from images often produces implausible bodies that lean, float, or penetrate the floor. Such methods ignore the fact that bodies are typically supported by the scene. A physics engine can be used to enforce physical plausibility, but these are not differentiable, rely on unrealistic proxy bodies, and are difficult to integrate into existing optimization and learning frameworks. In contrast, we exploit novel intuitive-physics (IP) terms that can be inferred from a 3D SMPL body interacting with the scene. Inspired by biomechanics, we infer the pressure heatmap on the body, the Center of Pressure (CoP) from the heatmap, and the SMPL body's Center of Mass (CoM). With these, we develop IPMAN, to estimate a 3D body from a color image in a "stable" configuration by encouraging plausible floor contact and overlapping CoP and CoM. Our IP terms are intuitive, easy to implement, fast to compute, differentiable, and can be integrated into existing optimization and regression methods. We evaluate IPMAN on standard datasets and MoYo, a new dataset with synchronized multi-view images, ground-truth 3D bodies with complex poses, body-floor contact, CoM and pressure. IPMAN produces more plausible results than the state of the art, improving accuracy for static poses, while not hurting dynamic ones. Code and data are available for research at https://ipman.is.tue.mpg.de.

==> images/experiments/ipmano_qual_result.tex <==
\begin{figure*}[ht]
\centerline{
\includegraphics[width=\linewidth]{images/experiments/ipmano_qual_result_img.pdf}
}
\vspace{-0.1in}
\caption{Qualitative evaluation of \nameMethodO on \yogiIOI. In the first column, the input images of a subject doing yoga poses. The second and third blocks show the results of \smplifyXMC~\cite{Mueller:CVPR:2021} and \nameMethodO respectively. In each block, the first and second column show the estimated mesh projected onto the image and from a second view. The last images show the \newtext{estimated} pressure map with the \physCOM (in \textcolor{magenta}{pink}) and the \physCOP (in \textcolor{green}{green}). \newtext{Overlapping \physCOM and \physCOP indicates a stable pose.}
}
\vspace*{-0.1in}
\label{figure:ipmano_qual_result}
\end{figure*}

==> images/experiments/ipmanr_qual_result.tex <==
\begin{figure*}[ht]
\centerline{
\includegraphics[width=\linewidth]{images/experiments/ipmanr_qual_result_img.pdf}
}
\vspace{-0.1in}
\caption{Qualitative evaluation of \nameMethodR on \rich. The first column shows the input images of a subject doing various sports poses. The second and third block of columns show the results of the \hmr (baseline) and \nameMethodR respectively. In each block, the first image shows the estimated mesh overlayed on the image, \newtext{the second image shows the estimated mesh in the world frame and the last image shows the \newtext{estimated} pressure map with the \physCOM (in \textcolor{magenta}{pink}) and the \physCOP (in \textcolor{green}{green}).}
}
\vspace*{-0.1in}
\label{figure:ipmanr_qual_result}
\end{figure*}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
